CausalGPS: An R Package for Causal Inference With Continuous Exposures

Quantifying the causal effects of continuous exposures on outcomes of interest is critical for social, economic, health, and medical research. However, most existing software packages focus on binary exposures. We develop the CausalGPS R package that implements a collection of algorithms to provide algorithmic solutions for causal inference with continuous exposures. CausalGPS implements a causal inference workflow, with algorithms based on generalized propensity scores (GPS) as the core, extending propensity scores (the probability of a unit being exposed given pre-exposure covariates) from binary to continuous exposures. As the first step, the package implements efficient and flexible estimations of the GPS, allowing multiple user-specified modeling options. As the second step, the package provides two ways to adjust for confounding: weighting and matching, generating weighted and matched data sets, respectively. Lastly, the package provides built-in functions to fit flexible parametric, semi-parametric, or non-parametric regression models on the weighted or matched data to estimate the exposure-response function relating the outcome with the exposures. The computationally intensive tasks are implemented in C++, and efficient shared-memory parallelization is achieved by OpenMP API. This paper outlines the main components of the CausalGPS R package and demonstrates its application to assess the effect of long-term exposure to PM2.5 on educational attainment using zip code-level data from the contiguous United States from 2000-2016.

==> illustration.tex <==
\section{Illustrations} \label{sec:illustrations}

For a simple illustration of basic Poisson and NB count regression the
\code{quine} data from the \pkg{MASS} package is used. This provides the number
of \code{Days} that children were absent from school in Australia in a
particular year, along with several covariates that can be employed as regressors.
The data can be loaded by
%
\begin{CodeChunk}
\begin{CodeInput}
R> data("quine", package = "MASS")
\end{CodeInput}
\end{CodeChunk}
%
and a basic frequency distribution of the response variable is displayed in
Figure~\ref{fig:quine}.

\begin{leftbar}
For code input and output, the style files provide dedicated environments.
Either the ``agnostic'' \verb|{CodeInput}| and \verb|{CodeOutput}| can be used
or, equivalently, the environments \verb|{Sinput}| and \verb|{Soutput}| as
produced by \fct{Sweave} or \pkg{knitr} when using the \code{render_sweave()}
hook. Please make sure that all code is properly spaced, e.g., using
\code{y = a + b * x} and \emph{not} \code{y=a+b*x}. Moreover, code input should
use ``the usual'' command prompt in the respective software system. For
\proglang{R} code, the prompt \code{"R> "} should be used with \code{"+  "} as
the continuation prompt. Generally, comments within the code chunks should be
avoided -- and made in the regular {\LaTeX} text instead. Finally, empty lines
before and after code input/output should be avoided (see above).
\end{leftbar}

\begin{figure}[t!]
\centering
\includegraphics{article-visualization}
\caption{\label{fig:quine} Frequency distribution for number of days absent
from school.}
\end{figure}

As a first model for the \code{quine} data, we fit the basic Poisson regression
model. (Note that JSS prefers when the second line of code is indented by two
spaces.)
%
\begin{CodeChunk}
\begin{CodeInput}
R> m_pois <- glm(Days ~ (Eth + Sex + Age + Lrn)^2, data = quine,
+    family = poisson)
\end{CodeInput}
\end{CodeChunk}
%
To account for potential overdispersion we also consider a negative binomial
GLM.
%
\begin{CodeChunk}
\begin{CodeInput}
R> library("MASS")
R> m_nbin <- glm.nb(Days ~ (Eth + Sex + Age + Lrn)^2, data = quine)
\end{CodeInput}
\end{CodeChunk}
%
In a comparison with the BIC the latter model is clearly preferred.
%
\begin{CodeChunk}
\begin{CodeInput}
R> BIC(m_pois, m_nbin)
\end{CodeInput}
\begin{CodeOutput}
       df      BIC
m_pois 18 2046.851
m_nbin 19 1157.235
\end{CodeOutput}
\end{CodeChunk}
%
Hence, the full summary of that model is shown below.
%
\begin{CodeChunk}
\begin{CodeInput}
R> summary(m_nbin)
\end{CodeInput}
\begin{CodeOutput}
Call:
glm.nb(formula = Days ~ (Eth + Sex + Age + Lrn)^2, data = quine, 
    init.theta = 1.60364105, link = log)

Deviance Residuals: 
    Min       1Q   Median       3Q      Max  
-3.0857  -0.8306  -0.2620   0.4282   2.0898  

Coefficients: (1 not defined because of singularities)
            Estimate Std. Error z value Pr(>|z|)    
(Intercept)  3.00155    0.33709   8.904  < 2e-16 ***
EthN        -0.24591    0.39135  -0.628  0.52977    
SexM        -0.77181    0.38021  -2.030  0.04236 *  
AgeF1       -0.02546    0.41615  -0.061  0.95121    
AgeF2       -0.54884    0.54393  -1.009  0.31296    
AgeF3       -0.25735    0.40558  -0.635  0.52574    
LrnSL        0.38919    0.48421   0.804  0.42153    
EthN:SexM    0.36240    0.29430   1.231  0.21818    
EthN:AgeF1  -0.70000    0.43646  -1.604  0.10876    
EthN:AgeF2  -1.23283    0.42962  -2.870  0.00411 ** 
EthN:AgeF3   0.04721    0.44883   0.105  0.91622    
EthN:LrnSL   0.06847    0.34040   0.201  0.84059    
SexM:AgeF1   0.02257    0.47360   0.048  0.96198    
SexM:AgeF2   1.55330    0.51325   3.026  0.00247 ** 
SexM:AgeF3   1.25227    0.45539   2.750  0.00596 ** 
SexM:LrnSL   0.07187    0.40805   0.176  0.86019    
AgeF1:LrnSL -0.43101    0.47948  -0.899  0.36870    
AgeF2:LrnSL  0.52074    0.48567   1.072  0.28363    
AgeF3:LrnSL       NA         NA      NA       NA    
---
Signif. codes:  0 '***' 0.001 '**' 0.01 '*' 0.05 '.' 0.1 ' ' 1

(Dispersion parameter for Negative Binomial(1.6036) family taken to be 1)

    Null deviance: 235.23  on 145  degrees of freedom
Residual deviance: 167.53  on 128  degrees of freedom
AIC: 1100.5

Number of Fisher Scoring iterations: 1


              Theta:  1.604 
          Std. Err.:  0.214 

 2 x log-likelihood:  -1062.546 
\end{CodeOutput}
\end{CodeChunk}

